PoseGPT: Quantization-based 3D Human Motion Generation and Forecasting

We address the problem of action-conditioned generation of human motion sequences. Existing work falls into two categories: forecast models conditioned on observed past motions, or generative models conditioned on action labels and duration only. In contrast, we generate motion conditioned on observations of arbitrary length, including none. To solve this generalized problem, we propose PoseGPT, an auto-regressive transformer-based approach which internally compresses human motion into quantized latent sequences. An auto-encoder first maps human motion to latent index sequences in a discrete space, and vice-versa. Inspired by the Generative Pretrained Transformer (GPT), we propose to train a GPT-like model for next-index prediction in that space; this allows PoseGPT to output distributions on possible futures, with or without conditioning on past motion. The discrete and compressed nature of the latent space allows the GPT-like model to focus on long-range signal, as it removes low-level redundancy in the input signal. Predicting discrete indices also alleviates the common pitfall of predicting averaged poses, a typical failure case when regressing continuous values, as the average of discrete targets is not a target itself. Our experimental results show that our proposed approach achieves state-of-the-art results on HumanAct12, a standard but small scale dataset, as well as on BABEL, a recent large scale MoCap dataset, and on GRAB, a human-object interactions dataset.

==> plots/pgf_read_table.tex <==
\pgfplotstableread{
D2_K1_C		D2_K1_pve	D2_K1_kl	D2_K1_AR	D2_K1_AS        D2_K1_FID  D2_K1_gnll    D2_K1_gbits
128		60.1		224		30.9		20.3		4.3	   2.5           115.4
256		52.1		256		33.5		21.2            3.5        3.0           138.5
512		49.73		288		33.6		21.1            3.7        3.3           152.3
}{\map}

\pgfplotstableread{
D2_K2_C         D2_K2_pve       D2_K2_kl        D2_K2_AR        D2_K2_AS        D2_K2_FID  D2_K2_gnll  D2_K2_gbits
128		40.18		384		28.5		20.3		3.2        2.4         221.6
256		38.3		448		29.4            20.8		2.8        2.5         230.8
512		33.8		512		29.6            21.4            2.9        3.3         304.7
}{\map}


\pgfplotstableread{
D2_K4_C         D2_K4_pve       D2_K4_kl	D2_K4_AR        D2_K4_AS	D2_K4_FID  D2_K4_gnll  D2_K4_gbits
128		       30.64		640		28.6		21.6            2.9        2.0         369.3
256		       28.15		768		27.0		21.0            2.7        2.3         424.7
512		27.3		896		27.1		20.9            2.5        2.5         461.7
}{\map}

\pgfplotstableread{
D2_K8_C         D2_K8_pve       D2_K8_kl	D2_K8_AR        D2_K8_AS        D2_K8_FID  D2_K8_gnll   D2_K8_gbits
128		27.17		1024		16.4		16.8		3.0  	   1.5 		554.0
256		23.65		1280		16.7		15.5		4.4  	   1.6 		590.9
512		26.65		1536		13.9		15.9		4.3  	   1.8 		664.8
}{\map}

\pgfplotstableread{
D2_C256_K       D2_C256_pve D2_C256_kl      D2_C256_AR D2_C256_ARN     D2_C256_AS  D2_C256_ASN    D2_C256_FID
1		        52.1		256             27.6        0.811  	        20.1        0.591            3.9
2		        38.3		448		        21.1        0.620           18.8         0.552   	    2.9
4		        28.15		736		       19.2         0.564   	    19.4         0.570          3.3
8               23.65		1280	       10.7         0.314   	    15.4	     0.452          4.4

}{\map}		

\pgfplotstableread{
D4_C256_K       D4_C256_pve     D4_C256_kl      D4_C256_AR  D4_C256_ARN     D4_C256_AS  D4_C256_ASN     D4_C256_FID D4_C256_gnll D4_C256_gbits
2		        50.7		    224		        32.0        0.941		    21.5	0.632	3.2         3.0          138.5
4		        35.5		    384		        31.8        0.935		    22.7	0.668	3.1         2.6          240.1
8               23.7	        640		       28.84	    0.848           21.6	0.635 	2.5         2.0          369.3
}{\map}		

\pgfplotstableread{
D8_C256_K       D8_C256_pve     D8_C256_kl      D8_C256_AR D8_C256_ARN	D8_C256_AS D8_C256_ASN	D8_C256_FID  D8_C256_gnll  D8_C256_gbits
2		        65.6		        112             28.8	0.847	    20.2	    0.594	      3.6          2.3           212.4
4		        47.52		        192		        31.8	0.935	    22.4	    0.658	    3.2          3.3           76.2
8               37.48		        320		        26.1	0.767	    20.3	    0.597	    3.1          2.8           129.3
}{\map}		
	

\pgfplotstableread{
D2_K    D2_C    	D2_pve	D2_kl	D2_AR D2_ARN D2_AS  D2_ASN      D2_FID      D2_gnll     D2_gbits
  1      128	        60.1	224	30.9	0.918  20.3	 0.597       4.3	 2.5         115.4
 1      256	            52.1    256	33.5	0.985  21.2  0.623      3.5      3.0         138.5
 1      512	            49.73   288	33.6	0.988  21.1  0.620      3.7      3.3         152.3
 2      128		        40.18   384	28.5	0.838  20.3	 0.597       3.2      2.4         221.6
 2      256		        38.3    448	29.4    0.864  20.8	 0.611       2.8      2.5         230.8
 2      512		        33.8    512	29.6    0.870  21.4  0.629      2.9      3.3         304.7
 4      128	        	30.64   640	28.6    0.841  21.6  0.635      2.9      2.0         369.3
 4      256		        28.15   768	27.0    0.794  21.0  0.617      2.7      2.3         424.7
 4      512		        27.3    896	27.1    0.797  20.9  0.614      2.5      2.5         461.7


}{\map}

\pgfplotstableread{
D2_C128_K    D2_C128_pve	D2_C128_kl	D2_C128_AR	D2_C128_AS      D2_C128_FID  D2_C128_gnll D2_C128_gbits
 1           60.1		224		30.9		20.3	        4.3	 2.5           115.4
 2           40.18		384		28.5		20.3		3.2      2.4         221.6
 4           30.64		640		28.6		21.6            2.9     2.0         369.3
}{\map}

\pgfplotstableread{
D2_C256_K    D2_C256_pve	D2_C256_kl	D2_C256_AR	D2_C256_AS      D2_C256_FID  D2_C256_gnll D2_C256_gbits
 1      	52.1		256		33.5		21.2            3.5          3.0          138.5
 2      	38.3		448		29.4            20.8		2.8          2.5          230.8
 4      	28.15		768		27.0		21.0            2.7          2.3          424.7
}{\map}

\pgfplotstableread{
D2_C512_K    D2_C512_pve	D2_C512_kl	D2_C512_AR	D2_C512_AS      D2_C512_FID    D2_C512_gnll D2_C512_gbits
 1      	49.73		288		33.6		21.1            3.7            3.3          152.3
 2      	33.8		512		29.6            21.4            2.9            3.3          304.7
 4      	27.3		896		27.1		20.9            2.5            2.5          461.7
}{\map}







